Sign Language Sense Disambiguation

This project explores methods to enhance sign language translation of German sign language, specifically focusing on disambiguation of homonyms. Sign language is ambiguous and understudied which is the basis for our experiments. We approach the improvement by training transformer-based models on various bodypart representations to shift the focus on said bodypart. To determine the impact of, e.g., the hand or mouth representations, we experiment with different combinations. The results show that focusing on the mouth increases the performance in small dataset settings while shifting the focus on the hands retrieves better results in larger dataset settings. Our results contribute to better accessibility for non-hearing persons by improving the systems powering digital assistants, enabling a more accurate interaction. The code for this project can be found on GitHub.

==> sections/dataset.tex <==
% We are using the same dataset as \citet{Camgöz2020Sign} for training and evaluation the transformer: 
We are using the RWTH-PHOENIX-Weather Database of German Sign Language \cite{Koller2015Continuous} for training and evaluation the transformer. This dataset contains videos of sign language speakers translating the weather forecast shown by the German TV channel PHOENIX and their translations. For 266 of the included sentences, the position of the face and the hands have been annotated. We use this portion of the data to produce a dataset fitted to test the hypothesis that incorporating more information about different body parts improves the disambiguation of homonyms. We focus on the videos which have annotations for hand and face tracking to correctly extract the hands and face from the videos. This procedure ensures that the input for our experiments is based on gold standard and prevents incorrectly extracted body parts.

\subsection{Baseline Data}
We preprocess the 266 sentences in such a way that it is formatted as a suitable input for the transformer model. We extracted the following information from the available metadata: video name, video representation, signer, gloss and text (spoken language sentence). The video representation is a tensor of the pillow \cite{clark2015pillow} representations of the singular frames.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/bodypart_extraction_example.png}
    \caption{Example for body part extraction.}
    \label{fig:bodypart_pics}
\end{figure}

\subsection{Body Part Extraction}
We want to enhance the recognition of ambiguous sentences by manually shifting the transformer's focus on different body parts.
We do this by additionally feeding the tensors of the extracted body parts into the transformer at training time. \\
We extract the body parts by the coordinates provided by the dataset \cite{Koller2015Continuous} to locate the positions of the right hand, left hand and the nose. We extract them with the pillow Python package \cite{clark2015pillow}. An example image and the cropped frames can be seen in Figure \ref{fig:bodypart_pics}. \\
With the cut-outs of the bodyparts, we then went through the same procedure as for our baseline data and create datasets in addition to our baseline data for the following combinations:
\begin{itemize}
    %\item Mouth only
    %\item Both hands only
    \item Mouth and whole picture
    \item Both hands and whole picture
    \item Mouth, both hands and whole picture
\end{itemize}
The bodypart data thus contains the same meta data as the baseline data, except for the image representations. To create a joint representation of the information coming from multiple pictures, we multiplied the vectors. This keeps the dimensionality the same, but adds the additional information. \\





==> sections/experiment.tex <==
\subsection{Task Definition}
\label{sec:taskdef}
There are two relevant tasks for our project which must be distinguished.
Sign language recognition means extracting the conveyed information and assigning the individual signs in a sequence matching glosses. In contrast, sign language translation is the generation of a spoken language text that transports the same meaning as the original sign language sentence.
While both tasks share similarities, it is important to distinguish them. The transformer employed in our project performs recognition and translation jointly, but we focus on improving only the improving the translation task.


% \subsection{Testing and Pre-Evaluation with BLIP Toy Example}
% The hypothesis that we want to prove with our experiment is that incorporating different body parts like the mouth in the input of a model can help to disambiguate sign language.\\
% To test this hypothesis, we first try a small example on BlipForImageTextRetrieval \cite{Li2022BLIP} which is a pretrained transformer that measures the probability that a given image matches a given text. We use three images as input, representing the ambiguous German sign "jam"/"color" (see figure \ref{fig:marmelade}). Two of the images show the sign produced with mouthing, one of them doesn't. The model should produce the probability for each of the images matching the same text "sign for the word jam". Surprisingly, the image of the sign with mouthing of the word "color" has the highest probability with 98\%, followed by the image without mouthing with 96\% and the image of the sign for the word "jam" with mouthing with 95\%. This small example shows that a pretrained transformer for standard image retrieval cannot distinguish very well between ambiguous signs and cannot solve them either. It does work in a way of recognizing an image of a sign in general. This demonstrates the current state of disambiguation of sign language and the importance of enhancing models in this field.
% \begin{figure}    
% \includegraphics[width=\textwidth/2]{img/image_examples.png}
%     \caption{Input images for BlipForImageRetrieval. Left: german sign for "jam" with mouthing; middle: german sign for "color" with mouthing; right: german sign for "jam"/"color" without mouthing}
%     \label{fig:marmelade}
% \end{figure}

%\ozge{in general the skeleton of the paper looks really nice!}

\subsection{Signjoey - Sign Language Transformer}
\label{sec:experiment2}
\colorbox{green}{TODO: ctc part just as an idea, should be revised}
Our transformer setup is based on the work by \citet{Camgöz2020Sign}, which introduced a unified transformer architecture for both sign language recognition and translation tasks. This architecture builds upon the Joey NMT framework \citep{kreutzer-etal-2019-joey}, leveraging the Connectionist Temporal Classification (CTC) loss function to enable joint learning and training in an end-to-end manner. The CTC loss function addresses the challenge of ground-truth timing information, often missing in unsegmented time-series data such as videos or audio sequences. In our context, this means we do not have precise information about when each sign begins and ends within a video. Accurate timing information is crucial for correctly labeling sequences in time-series data, which is essential for training sign language recognition models that rely on supervised learning. The CTC introduces an augmented output space:

\[
L' = L \cup \{ \epsilon \}
\]

where \( \epsilon \) is a "blank" label used to handle variable input lengths.\\


At each time step \( t \), the model generates a probability distribution over the augmented output space \( L' \). 

\[
y_t = \{ p(y_t = l \mid x), \; l \in L' \}
\]

where \( y_t \) is the model’s output probability distribution at time step \( t \) over \( L' \), and \( l \) represents each label in the augmented output space. \\


The loss function, \( L_{CTC} \), sums over all possible alignments between the input sequence \( x \) and the target labels \( z = (z_1, z_2, \ldots, z_U) \). 
\[
L_{CTC} = - \log P(z \mid x)
\]

where \( z \) is the target sequence that the model aims to predict. \\

It uses the output probabilities over \( L' \) to compute the probability of the target sequence \( z \) by summing over all possible alignments of \( z \) with the input sequence \( x \).\\

We explore different hyperparameter spaces as listed in Table \ref{tab:Hyperparameters}. As the hyperparameter have a big influence on the results, we change them accordingly to the reported experiment.
% We start our experiments with the configuration provided by \citet{Camgöz2020Sign}:

\begin{table}[h!]
    \centering
    \footnotesize
    \begin{tabular}{|c|c c c|} \hline 
         \textbf{Params} & \textbf{Values} & & \\ \hline 
         Epochs & 5 & 10 & 20 \\ \hline
         Hidden Dims & 256 & 512 & \\ \hline
         Batch Size & 16 & 32 & 64\\ \hline 
         Learning Rate (LR) & \(1 \times 10^{-3}\) & \(1 \times 10^{-4}\) & \(1 \times 10^{-5}\) \\ \hline 
    \end{tabular}
    \caption{Hyperparameter Setting}
    \label{tab:Hyperparameters}
\end{table}

% As our experiments progressed, we expanded our hyperparameter search space to balance the needs of our datasets with the capabilities of the transformer architecture. We aimed to address issues related to data limitations as thoroughly as possible. For more details, see the section on Experimental Setup and Evaluation Results.


